The $s$-value: evaluating stability with respect to distributional shifts

Common statistical measures of uncertainty such as $p$-values and confidence intervals quantify the uncertainty due to sampling, that is, the uncertainty due to not observing the full population. However, sampling is not the only source of uncertainty. In practice, distributions change between locations and across time. This makes it difficult to gather knowledge that transfers across data sets. We propose a measure of instability that quantifies the distributional instability of a statistical parameter with respect to Kullback-Leibler divergence, that is, the sensitivity of the parameter under general distributional perturbations within a Kullback-Leibler divergence ball. In addition, we quantify the instability of parameters with respect to directional or variable-specific shifts. Measuring instability with respect to directional shifts can be used to detect the type of shifts a parameter is sensitive to. We discuss how such knowledge can inform data collection for improved estimation of statistical parameters under shifted distributions. We evaluate the performance of the proposed measure on real data and show that it can elucidate the distributional instability of a parameter with respect to certain shifts and can be used to improve estimation accuracy under shifted distributions.

==> sections/0-abstract.tex <==
% -*- Mode: latex -*- %


Common statistical measures of uncertainty such as $p$-values and confidence intervals quantify the uncertainty due to sampling, that is, the uncertainty due to not observing the full population. However, sampling is not the only source of uncertainty. In practice, distributions change between locations and across time. This makes it difficult to gather knowledge that transfers across data sets. We propose a measure of instability that quantifies the distributional instability of a statistical parameter with respect to Kullback-Leibler divergence, that is, the sensitivity of the parameter under general distributional perturbations within a Kullback-Leibler divergence ball. In addition, we quantify the instability of parameters with respect to directional or variable-specific shifts. Measuring instability with respect to directional shifts can be used to detect under which kind of distribution shifts a statistical conclusion might be reversed. We discuss how such knowledge can inform data collection for transfer learning of statistical parameters under shifted distributions. We evaluate the performance of the proposed measure on real data and show that it can elucidate the distributional instability of a parameter with respect to certain shifts and can be used to improve estimation accuracy under shifted distributions.

%Common statistical measures like $p$-values and confidence intervals quantify the uncertainty due to sampling, that is, the uncertainty due to not observing the full population. In practice, populations change between locations and across time. This makes it difficult to gather knowledge that transfers across data sets. We propose a measure of stability that quantifies the distributional instability or uncertainty of a statistical estimand with respect to Kullback-Leibler divergence, that is, the sensitivity of the parameter under general distributional perturbations within a Kullback-Leibler divergence ball. However, often not all aspects of distribution change. Hence, we also propose measures to estimate the stability of parameters with respect to directional or variable-specific shifts.  
%
%
%Further, we demonstrate how the measure of distributional uncertainty can be used to prioritize data collection for better estimation of statistical parameters under shifted distribution. We evaluate the performance of the proposed measure in simulations and real data and show that it can elucidate the distributional (in-)stability of an estimator with respect to certain shifts and give more accurate estimates of parameters under shifted distribution with limited information such as summary statistics of certain covariates.


% Further, we introduce a transfer learning technique that allows to obtain better estimates of statistical parameters or predictive model under shifted distribution when limited information such as summary statistics of covariates or only few samples are available from the shifted distribution. \Dominik{remove/rewrite the transfer learning stuff to reflect our new focus. "We demonstrate how the method can be to prioritize data collection for transfer learning"}
%We evaluate the performance of the proposed measure in simulations and show that it can elucidate the distributional (in-)stability of an estimator with respect to certain shifts and give more accurate estimates of parameters under shifted distribution with limited information.



%old abstract

%Common statistical measures of uncertainty like $p$-values and confidence intervals quantify the uncertainty due to sampling, that is, the uncertainty due to not observing the full population. In practice, populations change between locations and across time. This makes it difficult to gather knowledge that transfers across data sets. We propose a measure of uncertainty that quantifies the distributional uncertainty of a statistical estimand with respect to Kullback-Leibler divergence, that is, the sensitivity of the parameter under general distributional perturbations within a Kullback-Leibler divergence ball. If the signal-to-noise ratio is small,
% %close to the detection threshold, 
% distributional uncertainty is a monotonous transformation of the signal-to-noise ratio. In general, however, it is a different concept and corresponds to a different research question. Further, we propose measures to estimate the stability of parameters with respect to directional or variable-specific shifts.  
%We also demonstrate how the measure of distributional uncertainty can be used to prioritize data collection for better estimation of statistical parameters under shifted distribution. We evaluate the performance of the proposed measure in simulations and real data and show that it can elucidate the distributional (in-)stability of an estimator with respect to certain shifts and give more accurate estimates of parameters under shifted distribution with limited information such as, summary statistics of certain covariates.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../mainnew.tex"
%%% End:


==> sections/3-Applications.tex <==





% \section{Applications}

% \Dominik{I am thinking that we might want to delete all but the most exciting applications and move it up before the finite-sample and optimization results? It is important to get the reader interested and excited before diving into particularities how we solve the problem.}
% \subsection{Confounding}
% We will see that the stability measure $r$ can be used to evaluate sensitivity with respect to confounding. The population mixture may change across settings which may hamper the replicability of findings. For example,  it is often hard to say if the findings from a study performed in United States, which has a diverse mix of ethnicity will hold in Asia, say. It then becomes useful to quantify the minimum change in the mixture weights that will swap the findings, which we illustrate in the corollary below.

% \begin{corollary}
% Consider a mixture of $m$ distributions $\{P_i\}_{i=1}^m$ given by ${P} = \sum c_i {P}_i$, with weights $c_i \ge 0$ and $\sum c_i =1$. Consider another mixture of distributions ${P}' = \sum c_i' {P}_i$ for some  weights $c_i' \ge 0$ with $\sum c_i' =1$. For a parameter of interest $\theta$, let the weights satisfy
% \begin{equation*}
%   \max_i \log(c_i'/c_i) \le r( \theta, P,0).
% \end{equation*} 
% Then we have,
% \begin{equation*}
% \mathrm{sign}(\theta(P)) = \mathrm{sign}(\theta(P')).
% \end{equation*}
% \end{corollary}
% \begin{proof}
% By assumption, we have
% \begin{equation*}
%     D({P}' \| {P}) \le r( \theta, P,0) .
% \end{equation*}
% Thus, by Theorem~\ref{thm:Donsker-Varadhan},  we have $\mathrm{sign}(\theta(P)) = \mathrm{sign}(\theta(P'))$.
% \end{proof}
% This result allows to easily interpret values of $r$ in terms of how results would change if mixture components of the distribution change. Note that this is a conservative result and that the class

% \begin{equation}
%     \{ {P'}: D({P}' \| {P}) \le r(\theta,{P},0) \}
% \end{equation}
% is much larger than the class considered in the corollary.

% A special case is $\epsilon$-contamination. In that case, ${P}=(1-\epsilon){P}_1 + \epsilon {P}_2$ and ${P}' = {P}_1$. This case is related to robust statistics. The difference is that both training and test data can be contaminated in our case. Classical approach: remove outliers and fit on uncontaminated distribution. Different pre-processing pipelines can lead to very different results! One way to introduce heterogeneity is simply to compare across different pre-processing pipelines: cut outliers at different thresholds, remove two principal components instead of one,...
% \Suyash{But if I do not know the change in contaminated proportion, how do I use the r-value I report?} \Dominik{You could use indicator variables for different batches and tilt in that direction}

% \subsection{Errors-in-variables}
% As before, let $Z$ be a random variable having distribution $G_0$, which is contaminated by an error variable $\epsilon$ having distribution $F$ such that $Z+\epsilon$ has distribution $P =G_0*F$. Again as before, we have a parameter of interest $\theta$. We are interested in understanding the stability of the parameter when the noise distribution shifts from $F$ to $F'$ resulting in the shift in distribution, $P_0$ to $P'=G_0*F'$.


% Then, due to convexity of the KL-divergence,
% \begin{equation*}
%     D_{KL}(P \|  P') \le D_{KL}(F \|  F').
% \end{equation*}
% Thus, we have the following corollary.

% \begin{corollary}
% Let
% \begin{equation*}
%   D(P \|  P') \le r(\theta, P).
% \end{equation*} 
% Then,
% \begin{equation*}
% \mathrm{sign}(\theta(P)) = \mathrm{sign}(\theta(P')).
% \end{equation*}
% \end{corollary}
% In words, if the change in distributions of the measurement error does not exceed $r(\cdot)$, the sign of $\theta(P)$ does not change.



% \subsection{Example: invariance}

% In which cases is the tilted expectation the same as the original expectation? 
% The distribution factorizes as follows:
% \begin{equation*}
%    p(y,z,o) = p(y,o|z)  p(z)
% \end{equation*}
% We want to replace this distribution with
% \begin{equation*}
%     p(y,o |z) p^*(z),
% \end{equation*}
% where $p^*$ is an adversarially chosen distribution. If $X= f(Y,O)$ and
% \begin{equation}
%     \mathbb{E}[X|Z] = \mathbb{E}[X],
% \end{equation}
% then
% \begin{equation}
% \mathbb{E}^*[X] = \mathbb{E}[X]
% \end{equation}
% for all choices of $p^*(z)$. The proof is simple:
% \begin{equation}
%     \mathbb{E}^*[X] = \mathbb{E}^*[\mathbb{E}^*[X|Z]] = \mathbb{E}^*[\mathbb{E}[X|Z]] =\mathbb{E}^*[\mathbb{E}[X]] = \mathbb{E}[X].
% \end{equation}
% The reverse can also be shown. Thus,
% \begin{equation}
%     \mathbb{E}[X] = \mathbb{E}^*[X]
% \end{equation}
% for all densities $p^*(z) << p(z)$ if and only if
% \begin{equation}
%     \text{Var}(\mathbb{E}[X|Z]) = 0.
% \end{equation}

% \Suyash{Theoretically makes sense but in practise, we may have some variability consider section 9.3.}

% \Dominik{not enough time to properly write up invariance and causality}
% \subsection{Invariance and causality}

% Let's assume that we collect data $(X,Y)$ from different experimental conditions $E$. It has recently been shown that if a set of variable $S$ is causal for prediction of a response variable, then the conditional distributions
% \begin{equation}\label{eq:causalinvariance}
%     Y | X_S = x, E=e \text{ and } Y^f | X_S = x, E=f
% \end{equation}
% are equal across all environments $e,f$ that arise from interventions on the covariates. In particular, equation~\eqref{eq:causalinvariance} implies that
% \begin{equation*}
%     \mathbb{E}[Y | X_S = x , E=e] = \mathbb{E}[Y | X_S = x, E=f].
% \end{equation*}
% This can be reformulated in the following way. The random variable
% \begin{equation}
%   g(X,E) = \mathbb{E}[Y | X_S,E] - \mathbb{E}[Y | X_S]
% \end{equation}
% has invariant mean under distributional changes in $(X,E)$, i.e.\ its variance is zero. Invariant model vs 

% \Suyash{We still need to do this for each subset S. I was wondering how are we adding to already existing method (in a more efficient way)}


% \subsection{Example: dense dependency structures can hamper replicability and transferability of results across distributions}

% Consider the following conditional independence graph:

% \begin{center}
% \begin{tikzpicture}
%   [scale=.5,every node/.style={circle,fill=blue!20}]
%   \node (n6) at (1,10) {$E$};
%   \node (n4) at (4,8)  {$X_4$};
%   \node (n5) at (8,9)  {$X_5$};
%   \node (n1) at (11,8) {$X_1$};
%   \node (n2) at (9,6)  {$X_2$};
%   \node (n3) at (5,5)  {$X_3$};

%   \foreach \from/\to in {n6/n4,n4/n5,n5/n1,n2/n5,n2/n3,n3/n4}
%     \draw (\from) -- (\to);

% \end{tikzpicture}
% \end{center}
% The distribution $p(X_1|X_5)$ is invariant across environments, i.e.\
% \begin{equation}
%     p(X_1|X_5,E=e) = p(X_1|X_5,E=e')
% \end{equation}
% but in general $p(X_4,X_5)$ is not
% \begin{equation}
%     p(X_4,X_5 | E=e) \neq p(X_4,X_5 | E=e')
% \end{equation}
% On the other hand, let's consider a sparse graph:
% \begin{center}
% \begin{tikzpicture}
%   [scale=.5,every node/.style={circle,fill=blue!20}]
%   \node (n6) at (1,10) {$E$};
%   \node (n4) at (4,8)  {$X_4$};
%   \node (n5) at (8,9)  {$X_5$};
%   \node (n1) at (11,8) {$X_1$};
%   \node (n2) at (9,6)  {$X_2$};
%   \node (n3) at (5,5)  {$X_3$};

%   \foreach \from/\to in {n6/n4,n4/n5,n5/n1,n2/n3}
%     \draw (\from) -- (\to);
    
%     \end{tikzpicture}
% \end{center}
% Now there are a lot more quantities that are invariant across different conditional values $E=e$:
% \begin{equation}
%     p(X_3|X_2,E=e) = p(X_3|X_2,E=e')
% \end{equation}
% Thus, conditional distributional stability is in general related to the sparsity structure of the conditional independence graph. However, while conditional independence graphs can answer distributional replicability questions in special cases, conditional independence graphs can in general not answer the question whether a specific statistical functional is constant under conditioning or not. This insight can guide how we report and rank associations. Given the dependence structure, we might only want to report (conditional) associations that are stable under certain distributional changes. For example, above $p(X_1 | X_5)$ is invariant across settings $E=e$ while $p(X_5|X_1)$ is not. More specifically,
% \begin{equation}
%     p(X_5 | X_1,E=e) \neq p(X_5 | X_1,E=e')
% \end{equation}
% while
% \begin{equation}
%     p(X_1 | X_5,E=e) = p(X_1 | X_5,E=e').
%   \end{equation}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../mainnew.tex"
%%% End:


==> sections/4-consistency-optimization.tex <==
\section{Consistency results}
\begin{assumption}
\label{ass:worst-if-consistency}
Let $Q_n$ be the distribution function as returned by Algorithm~\ref{alg:r-M} at convergence and let $Q_0$ be the worst distribution under the population. $Q_n$ satisfies the following consistency property:
\begin{align*}
\mathbb{E}_{P_0}[(e^{\lambda_n \phi(Z, Q_n)}-e^{\lambda_0 \phi(Z, Q_0)})^2] = o\left(\frac{1}{n}\right),
\end{align*}
where $\phi$ is the influence function of the parameter.
\end{assumption}
%\begin{lemma}
%With $\lambda_n=\argmin_{\lambda}\mathbb{E}_{P_n}[e^{\lambda \phi(Z,Q_n)}]$, we have under assumption~\ref{ass:worst-if-consistency} that $\sqrt{n}(\lambda_n -\lambda_0) =O_{P}(1),$ where $\lambda_0=\argmin_{\lambda}\mathbb{E}_{P_0}[e^{\lambda \phi(Z,Q_0)}]$.
%\end{lemma}

\begin{theorem}
\label{thm:asy-norm-general}
Under Assumption~\ref{ass:worst-if-consistency},  $r(\theta,P_n)$ is asymptotically normal,
\begin{align*}
\sqrt{n}(r(\theta,P_n)-r(\theta,P_0)) \overset{d}{\rightarrow} N(0,V),
\end{align*}
where $V=Var(e^{\lambda^* \phi(Z,Q_0)}).$
\end{theorem}


\section{Convergence Analysis}

\begin{proposition}
\label{thm:alg-convergence}
Parameter $\theta(P)$ decreases with each iteration and if we are in a local neighborhood of the optimal solution(even locally optimal), which is well separated from other optimal solutions, then the algorithm always converges to that optimal solution.
\end{proposition}
\begin{definition}
A probability distribution $R$ is said to be a locally optimal solution to problem \eqref{eqn:general-optim} if $\theta(R)=0$ and there exists a small $\epsilon>0$ such that $D_{KL}(R||P_0) \leq D_{KL}(P||P_0)$ for all $P:  \theta(P)=0 \hspace{0.1in} \text{and} \hspace{0.1in} D_{KL}(P||Q) <\epsilon$.
\end{definition}
\begin{theorem}
\label{thm:optim-result}
$\popt$ is a locally optimal solution to the problem \eqref{eqn:general-optim} if and only if $\popt$ is given by $d\popt(z)=e^{c \phi(z,\popt)}dP_0(z)$ for some constant $c$.
\end{theorem}
\begin{proposition}
Let $R^{k}_n$ be the sequence of probability distributions generated by the second stage of Algorithm~\ref{alg:r-M}. Then, we have:
\begin{enumerate}
\item The sequence $D_{KL}(R^k_n||P_n)$ is decreasing and converges.
\item Any limit point of the sequence $\{R^k_n\}_{k \geq 1}$ is a locally optimal solution to problem \eqref{eqn:general-optim}.
\end{enumerate}
\end{proposition}
%\begin{theorem}
%\label{thm:optim-result}
%Let $\popt$ be a locally optimal solution to the problem \eqref{eqn:general-optim}, i.e., in the neighborhood, it is closest to the training distribution, $P_0$ such that $\theta(\popt)=0$ and let $\phi(Z,P)$ be the influence function of parameter $\theta(P)$, then $\popt$ is given by $d\popt(z)=e^{c \phi(z,\popt)}dP_0(z)$ for some constant $c$.
%\end{theorem}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../mainnew.tex"
%%% End:


==> sections/6-r-value-M-est.tex <==
%\section{S-values of M-estimators}
\section{S-values of parameters defined via risk minimization}
\label{sec:multidim_M_est}

Here, we discuss how to compute $s$-values for parameters defined via risk minimization and generalize to multi-parameter settings. Let us describe two examples where this is of interest. First, for a parameter vector $\eta$, each component might correspond to the causal effect of a subgroup. One may then ask whether there is a small distribution shift that renders all causal effects zero. These theory outlined in this section is also relevant for settings where one is interested in a single parameter in the presence of nuisance parameters. For example, in causal inference one component of the parameter vector might corresponds to the causal effect of interest, while the other components of the vector might correspond to the effect of observed confounders, which are not of interest by themselves.

We consider the following setting. Let $\Theta \subseteq \mathbb{R}^p$ be the parameter (model) space, $P_0$ be the data generating distribution (training distribution) on the measure space $(\mathcal{Z},\mathcal{A})$, $Z$ be a random element of $\mathcal{Z}$, and $L: \Theta \times \mc{Z} \rightarrow \mathbb{R}$ be a loss function, which is strictly convex and differentiable in its first argument.
Define the parameter $\theta^M(P)$ for $P \in \mc{P}$ via
\begin{equation}
\label{eq:M-est}
  \theta^M(P) = \arg \min_{\theta \in \Theta} \E_{P}[L(\theta, Z)].
\end{equation}  
Let $\ell(\theta,Z) = \partial_{\theta} L(\theta, Z)$. So far, for simplicity we have only considered $s$-values of one-dimensional parameters. In practice, we need a slightly more general notion of $s$-values that can handle $p$-dimensional parameters. For $\eta \in \mathbb{R}^{p}$, define the extended $s$-value via
\begin{equation}\label{eq:4}
   s(\theta^M-\eta,P_0)=\sup_{P \in \mc{P}}\exp\{ -D_{KL}(P||P_0)\} \hspace{0.1in} \text{s.t.} \hspace{0.1in} \theta^M(P) - \eta = 0.
\end{equation}
Choosing $\eta$ is similar to choosing a null hypothesis for significance testing in statistical decision problems. For example, in linear regression it is common to test the global null, where the regression coefficient is assumed to be zero for all components. Analogously, in this setting one might ask whether just a small distributional shift can shift all components of the parameter to zero.

Similar to the one-dimensional mean case (Section \ref{sec:r-value-mean}), the $s$-value in \eqref{eq:4} can be obtained by solving a $p$-dimensional convex optimization problem that we state in the following corollary. Its proof can be found in Appendix~\ref{proof:r-values-m}.

\begin{corollary}\label{cor:r-values-m}
Let $\ell(\eta,Z)$ have a finite moment generating function on $\mathbb{R}^p$ under $P_{0}$ for all $\eta \in \Theta$. Then, the $s$-value of the parameter $\theta^M$ as defined in \eqref{eq:M-est} is given by
\begin{equation}
  s(\theta^M-\eta,P_0) = \inf_{\lambda \in \mathbb{R}^{p}} E_{P_0}[e^{\lambda^{\intercal} \ell(\eta,Z)}].
\end{equation}
\end{corollary}
Consistency and asymptotic normality can be obtained analogously as in Lemma~\ref{lem:asy-norm-mean} and Lemma~\ref{lem:asy-normality-mean}. A general theorem is formulated in the Appendix, Section~\ref{sec:proof-ci}.
We next present some examples of parameters defined via risk minimization.
%In words, we can tilt the parameter vector $\theta^M(P_{0}) = \eta_{0} \in \mathbb{R}^{p}$ to any other vector $\theta^M(P) = \eta \in \mathbb{R}^{p}$ by solving a $p$-dimensional convex optimization problem over $\lambda$.

\begin{example}[Regression]
Let $\mc{X} \subseteq \mathbb{R}^p$ be a $p$-dimensional feature space and $\mc{Y}$ be the space of response. Let $Y \in \mc{Y}$ satisfy $Y=X\theta+\epsilon$, where $\theta \in \Theta \subset \R^p$ and $\epsilon$ is uncorrelated with $X$. Then the OLS parameter $ \theta^M(P) $ is given by
\begin{align*}
\theta^M(P)= \argmin_{\theta} \E_{P}[(Y-X\theta)^2].
\end{align*}
If $X^{\intercal}(Y-X\eta)$ has finite moment generating function on $\mathbb{R}^p$ for all $\eta \in \Theta$ then using Corollary~\ref{cor:r-values-m}, we have
\begin{equation*}
 s(\theta^M-\eta,P_0) = \inf_{\lambda \in \mathbb{R}^{p}} \E_{P_0}[e^{\lambda^{\intercal} X^{\intercal} (Y - X \eta)}].
\end{equation*}



\end{example}

\begin{example}[Generalized linear models]
\label{exm:glm}
Let $\mc{X} \subseteq \mathbb{R}^p$ be a $p$-dimensional feature space and $\mc{Y}$ be the space of response. Let $Y \in \mc{Y}$ satisfy $\E[Y \mid X]=g^{-1}(X\theta)$ where $\theta \in \Theta \subset \R^p$ and $g$ is the link function. With slight abuse of notation, let $L(Y, X \theta) $ be the negative log-likelihood function. The maximum likelihood parameter $\theta^M$ is given by
\begin{align*}
\theta^M(P)= \argmin_{\theta} \E_{P}[L(Y,X\theta)].
\end{align*}

If $X^{\intercal}\partial_2 L(Y,X\eta)$ has finite moment generating function on $\mathbb{R}^p$ for all $\eta \in \Theta$ then using Corollary~\ref{cor:r-values-m}, we have
\begin{equation*}
 s(\theta^M-\eta,P_0) = \inf_{\lambda \in \mathbb{R}^{p}} \E_{P_0}[e^{\lambda^{\intercal} X^{\intercal}\partial_{2}L(Y,X\eta)}].
\end{equation*}
\end{example}


We next characterize directional $s$-values. We define the extended directional $s$-value as
\begin{equation}\label{eq:5}
   s_E(\theta^M-\eta,P_0)=\sup_{P \in \mc{P}, P[\bullet|E] = P_{0}[\bullet|E]}\exp\{- D_{KL}(P||P_0)\} \hspace{0.1in} \text{s.t.} \hspace{0.1in} \theta^M(P) - \eta = 0.
 \end{equation}
 Similarly as above, directional $s$-values can be obtained by solving a convex optimization problem that we state in the following corollary. We present the proof in Appendix~\ref{proof:r-values-m-cond}.
\begin{corollary}[Directional shifts]\label{cor:r-values-m-cond}

Let $\ell(\eta,Z)$ have a finite moment generating function on $\mathbb{R}^p$ under $P_{0}$. Then,
\begin{equation}
  s_E(\theta^M-\eta,P_0) = \inf_{\lambda } \E_{P_0}[ e^{ \lambda^{\intercal} E_{P_0}[\ell(Z,\eta)|E]}].
\end{equation}
\end{corollary}
Consistency and asymptotic normality can be obtained analogously as in Lemma~\ref{lem:consistency-mean-cond} and Lemma~\ref{lem:asy-normality-cmean}. A general theorem is formulated in the Appendix, Section~\ref{sec:proof-ci}.

Next, we present an example from regression setting. 
\begin{example}[Regression]
\label{exm:reg-dir}
Let $\mc{X} \subseteq \mathbb{R}^p$ be a $p$-dimensional feature space and $\mc{Y}$ be the space of the response. Let $Y \in \mc{Y}$ satisfy $Y=X\theta+\epsilon$, where $\theta \in \Theta \subset \R^p$ and $\epsilon$ is independent of $X$. As above, the OLS parameter $ \theta^M(P) $ is defined as
\begin{align*}
\theta^M(P)= \argmin_{\theta} \E_{P}[(Y-X\theta)^2].
\end{align*}
If $X^{\intercal}(Y-X\eta)$ has finite moment generating function on $\mathbb{R}^p$ for all $\eta \in \Theta$, then Corollary~\ref{cor:r-values-m-cond} implies 
\begin{equation*}
 s_X(\theta^M-\eta,P_0) = \inf_{\lambda \in \mathbb{R}^{p}} \E_{P_0}[e^{\lambda^{\intercal} X^{\intercal} (\mathbb{E}_{P_0}[Y|X] - X \eta)}].
\end{equation*}
Now let us investigate the case with high directional distributional stability with respect to $E=X$. In the following, let us assume that $s_X(\theta^M-\eta,P_{0}) = 0$ for all $\eta \neq \theta(P_{0})$ and that $X$ has positive density with respect to the Lebesgue measure. By definition of the $s$-value  we have $\theta^M(P) = \theta^M(P_{0})$ for every measure $P$ that is absolutely continuous with respect to $P_{0}$ and satisfies $P(\cdot|X=x) = P_{0}(\cdot|X=x)$ for all $x \in \mc{X}$. By definition of OLS, we must have that almost surely
\begin{equation*}
  \mathbb{E}_{P_0}[ X^{\intercal} (Y - X \theta^M)|X] = 0.
\end{equation*}
Thus, almost surely,
\begin{equation*}
 X^{\intercal} (\E_{P_{0}}[Y|X] - X \theta^M)=\mathbb{E}_{P_0}[ X^{\intercal} (Y - X \theta^M)|X] = 0.
\end{equation*}  
If $X$ has a density with respect to the Lebesgue measure, then $\E_{P_{0}}[Y|X] = X \theta^M$ almost surely. Thus, directional distributional instability in linear models with respect to $E=X$ is related to whether the linear model is a good approximation of the regression surface, i.e.\ $\E_{P_{0}}[Y|X] \approx X \theta^M$. More specifically, if the linear model is a good approximation of the regression surface, directional stability is high. This is an example, where distributional instability can be induced by model misspecification. As discussed earlier in Section~\ref{exm:anscombe}, distributional instability can also be induced by other sources such as the presence of exogenous covariates that are correlated both with covariates and the outcome.



\end{example}

We can similarly obtain results for generalized linear models (see Example \ref{exm:glm}).




\subsection{S-values for a single component}



In many cases, practitioners may be interested in obtaining the $s$-value for a single component of $\theta^M \in \R^p$ instead of the entire vector $\theta^M$. For example, in causal inference, one component of $\theta^M$ can correspond to average treatment effect while other parameters may not be of scientific interest. In such settings, one might want to evaluate the stability of the parameter of interest (the average treatment effect) and not the stability of the nuisance components. Let $\theta^M_k$ be the $k$-th component of parameter vector $\theta^M \in \R^p$ for $k \in \{1, \ldots, p\}$. 

Intuitively, to obtain the $s$-value of a single parameter, we seek for the smallest possible shift in distribution that tilts the parameter to a pre-determined value, hence, we take supremum over other remaining nuissance parameters. To be more precise, using the definition of $s$-values and Corollary \ref{cor:r-values-m}, we have
\begin{align}
  \label{eq:r-val-one-M}
  \begin{split}
  s(\theta^M_k-\eta_k,P_0) &= \sup_{P \in \mc{P}} \exp\{- D_{KL}(P||P_0)\} \text{ s.t. } \eta_k(P) -\eta_k = 0  \\
  &= \sup_{\eta_1, \ldots,\eta_{k-1},\eta_{k+1}, \ldots, \eta_p} \sup_{P \in \mc{P}} \exp\{- D_{KL}(P||P_0)\} \text{ s.t. } \eta(P) -\eta = 0 \\
  &= \sup_{\eta_1, \ldots,\eta_{k-1},\eta_{k+1}, \ldots, \eta_p} \inf_{\lambda \in \R^p} \E_{P_0}[ e^{ \lambda^{\intercal} \ell(\eta,Z)}].
  \end{split}
  \end{align}
% \begin{equation}
% \label{eq:r-val-one-M}
% s(\theta^M_k-\eta_k,P_0) =\sup_{\eta_1, \ldots,\eta_{k-1},\eta_{k+1}, \ldots, \eta_p} \inf_{\lambda \in \R^p} \E_{P_0}[ e^{ \lambda^{\intercal} \ell(\eta,Z)}].
% \end{equation}

 %\citet{Owen01} considers similar quantities as \eqref{eq:4} and \eqref{eq:r-val-one-M}. The author, however, investigates small (asymptotically negligible) shifts, and the algorithms to obtain estimates of $s$-values for single components as in \eqref{eq:r-val-one-M} do not come with any convergence guarantee for large shifts. The author also does not consider any form of directional shifts. 


We next obtain a finite sample estimate of $s$-values for individual components of $\theta^M$ and show that it is consistent to the population version. Let $P_n$ be the empirical distribution of $Z_i \overset{\text{i.i.d.}}{\sim} P_0$. We propose to estimate the $s$-value via the plugin estimator

\begin{align}
\label{eq:r-val-one-M-finite}
\begin{split}
\hat s(\theta^M_k-\eta_k,P_n) &=\sup_{\eta_1, \ldots,\eta_{k-1},\eta_{k+1}, \ldots, \eta_p} \inf_{\lambda \in \R^p} \E_{P_n}[ e^{ \lambda^{\intercal} \ell(\eta,Z)}] \\
&= \sup_{\eta_1, \ldots,\eta_{k-1},\eta_{k+1}, \ldots, \eta_p} \inf_{\lambda \in \R^p} \frac{1}{n} \sum_{i=1}^n e^{ \lambda^{\intercal} \ell(\eta,Z_i)}
\end{split}
\end{align}
%\begin{equation}
%\label{eq:r-val-one-M}
%\hat s(\theta_1,P_n,\eta_1) =\max_{\eta_2, \ldots, \eta_p} \min_{\lambda \in \R^p} E_{P_n}[ e^{ \lambda^{\intercal} \ell(\eta,Z)}].
%\end{equation}
This is a challenging optimization problem. The optimization problem in \eqref{eq:r-val-one-M-finite} is non-convex and hence, finding the global optimum in practice is intractable. In Appendix \ref{sec:r-value-general}, we propose algorithms to solve the optimization problem in \eqref{eq:r-val-one-M-finite} with convergence guarantees. We also propose a simple plug-in estimate in Appendix~\ref{sec:plug-in}. 

The non-convexity of the optimization problem has important consequences for interpreting $s$-values. For the sake of simplicity, let us assume that $n$ is large, that is that estimation errors due to finite samples can be ignored. If the estimated $s$-value is large, the algorithm constructs a small distribution shift that changes the sign of the parameter. In other words, the parameter is certifiably unstable. On the other hand, if the estimated $s$-value is small, then this could be due the algorithm being stuck in a local optimum. Thus, for non-convex problems a large $s$-value is an indication of instability, but a small $s$-value cannot be necessarily interpreted as a proof of stability. This is similar to hypothesis testing in statistical inference, where the non-significance of a $p$-value cannot be interpreted as a proof of the null hypothesis.


%We discuss some algorithms in Appendix \ref{sec:r-value-general}.

We next show consistency of $\hat s(\theta^M_k-\eta_k,P_n) $ to the corresponding population stability value $s(\theta^M_k-\eta_k,P_0)$. To this end, we make the following assumption.

% in Appendix Section \ref{sec:s-val-multi}.



%
%Let us now discuss how to estimate directional $s$-values of individual components. Suppose we want to obtain the directional $s$-value of the $k$-th component of vector $\theta^M \in \R^p$. Using Corollary \ref{cor:r-values-m-cond}, the population directional $s$-value is given by
%
%\begin{equation}
%\label{eq:r-val-one-M-cond}
%s_E(\theta^M_k-\eta_k,P_0) =\sup_{\eta_1, \ldots,\eta_{k-1},\eta_{k+1}, \ldots, \eta_p} \inf_{\lambda \in \R^p} E_{P_0}[ e^{ \lambda^{\intercal}\E_{P_0}[ \ell(\eta,Z)\mid E]}].
%\end{equation}













\begin{assumption}
\label{ass:uniform_convergence}
Let $\Sigma \subset \R^p$ be a compact subset such that the map $\eta \to \ell(\eta,Z)$ is continuous on $\Sigma$ and $\E_{P_0}[\sup_{\eta \in \Sigma}e^{\lambda^{\intercal}\ell(\eta,Z)}] < \infty$ for any $\lambda \in \R^p$. 
\end{assumption}

\begin{lemma}[Consistency of $s$-value]
\label{lem:consistency-one-comp}
Let $\Sigma_k$ denote the projection of $\Sigma$ on the $k$th co-ordinate. Under Assumption~\ref{ass:uniform_convergence}, we have $\sup_{\eta_k \in \Sigma_k}|\hat s(\theta^M_k-\eta_k,P_n)  -  s(\theta^M_k-\eta_k,P_0)| \overset{P}{\to} 0 $ for $k=\{1, \ldots, p\}$  as $n \to \infty$.
\end{lemma}
We present the proof of Lemma~\ref{lem:consistency-one-comp} in Appendix~\ref{proof:consistency-one-comp}.

\begin{example}[Regression]
Let $\mc{X} \subseteq \mathbb{R}^p$ be a $p$-dimensional bounded feature space and $\mc{Y}$ be the space of the response. Let $Y \in \mc{Y}$ satisfy $Y=X^{\intercal}\beta+\epsilon$, where $\beta \in \Theta \subset \R^p$ and $\epsilon$ is independent of $X$. 
We have $L(\eta,X,Y)=\frac{1}{2}(Y-X^{\intercal}\eta)^2$, $\ell(\eta, X,Y)=-X(Y-X^{\intercal}\eta)$ and hence, $\nabla_{\eta} \ell(\eta,X,Y)=XX^T$.
Now, for a compact subset $\Sigma \subset \R$, $\E_{P_0}[\sup_{\eta \in \Sigma}e^{\lambda^{\intercal}\ell(\eta,Z)}] < \infty$ if $\epsilon$ has a finite moment generating function on $\mathbb{R}$. Invoking Lemma~\ref{lem:consistency-one-comp}, we can conclude that the estimator is consistent.


Let us now discuss how to estimate directional $s$-values of individual components. Suppose we want to obtain the directional $s$-value of the $k$-th component of vector $\theta^M \in \R^p$. Using Corollary \ref{cor:r-values-m-cond}, the population directional $s$-value is given by

\begin{equation}
\label{eq:r-val-one-M-cond}
s_E(\theta^M_k-\eta_k,P_0) =\sup_{\eta_1, \ldots,\eta_{k-1},\eta_{k+1}, \ldots, \eta_p} \inf_{\lambda \in \R^p} E_{P_0}[ e^{ \lambda^{\intercal}\E_{P_0}[ \ell(\eta,Z)\mid E]}].
\end{equation}






\end{example}

Now we propose a finite sample estimator of the directional $s$-value of individual components and show consistency. 

%in Appendix Section \ref{sec:s-val-multi}.

Let $Q_n(\eta,E)$ be a finite sample estimator of $\E_{P_0}[ \ell(\eta,Z)\mid E]$, then the finite sample plugin estimator is given by
 \begin{equation}
\label{eq:r-val-one-M-finite-cond}
\hat s_E(\theta^M_k-\eta_k,P_n) =\sup_{\eta_1, \ldots,\eta_{k-1},\eta_{k+1}, \ldots, \eta_p} \inf_{\lambda \in \R^p} E_{P_n}[ e^{ \lambda^{\intercal} Q_{n}(\eta,E)}].
\end{equation}
Again, this is a challenging optimization problem. We discuss algorithms in Appendix \ref{sec:alg-cond-s}. A simplification that allows to derive upper bounds can be found in Appendix, Section~\ref{sec:plug-in}. 
We make the following additional assumption to show consistency of $\hat s_E(\theta^M_k-\eta_k,P_n)$.
\begin{assumption}
\label{ass:conditional-uniform-convergence}
 $\sup_{\eta} \sup_{e} \norm{ E_{P_{0}}[\ell(\eta,Z)|E=e] - Q_n(\eta,e)}_{\infty} \rightarrow 0$, where $Q_n(\eta,e)$ is an estimate of $E_{P_{0}}[\ell(\eta,Z)|E=e]$.
\end{assumption}
\begin{lemma}[Consistency of directional $s$-value]
\label{lem:consistency-one-comp-cond}
Under Assumptions~\ref{ass:uniform_convergence} and \ref{ass:conditional-uniform-convergence}, we have 
\begin{align*}
\sup_{\eta_k \in \Sigma_k}|\hat s_E(\theta^M_k-\eta_k,P_n)  -  s_E(\theta^M_k-\eta_k,P_0)| \overset{P}{\to} 0  \text{ for } k=\{1, \ldots, p\}
\end{align*}
 as $n \to \infty$.
%
%$\sup_{\lambda \in \Lambda} \sup_{\eta \in \Sigma} |E_{P_n}[ e^{ \lambda^{\intercal} Q(\eta,E)}]- E_{P_0}[ e^{ \lambda^{\intercal} E[\ell(\eta,Z)|E]}]| \overset{P}{\to} 0$.
\end{lemma}
We present the proof of Lemma~\ref{lem:consistency-one-comp-cond} in Appendix~\ref{proof:consistency-one-comp-cond}. To quantify uncertainty, in this settings we find the bootstrap preferrable over asymptotic expansions (as in Section~\ref{sec:r-value}) to account for the fact that the algorithm might get stuck in a local minimum.




